On partially wrapped Fukaya categories

We define a new class of symplectic objects called "stops", which roughly speaking are Liouville hypersurfaces in the boundary of a Liouville domain. Locally, these can be viewed as pages of a compatible open book. To a Liouville domain with a collection of disjoint stops, we assign an $A_\infty$-category called its partially wrapped Fukaya category. An exact Landau-Ginzburg model gives rise to a stop, and the corresponding partially wrapped Fukaya category is meant to agree with the Fukaya category one is supposed to assign to the Landau-Ginzburg model. As evidence, we prove a formula that relates these partially wrapped Fukaya categories to the wrapped Fukaya category of the underlying Liouville domain. This operation is mirror to removing a divisor. In v2, we also construct continuation functors without cascades, which should be of independent interest.

==> Appendices.tex <==
Let $\Sigma$ be a Riemann surface with boundary components $\partial_i\Sigma$, interior punctures $z_j$, and boundary punctures $\zeta^k$. Let $\epsilon_j$ be cylindrical ends at $z_j$, and likewise let $\epsilon^k$ be strip-like ends at $\zeta^k$, such that the images of the ends are pairwise disjoint.

Suppose further we are given a Liouville domain $(M,\lambda_M)$, and that $\partial_i\Sigma$ is labeled with a Lagrangian $L_i\hat M$. Additionally, we have a $\Sigma$-parametrized compatible Hamiltonian $\tild H$, a $\Sigma$-parametrized perturbing Hamiltonian $P$, along with a 1-forms $\beta$ with the following properties.
\begin{enumerate}
 \item\label{cd:translation invariant ends} On the cylindrical and strip-like ends, let $t$ be the coordinate of the compact $S^1$ or $[0,1]$ factor, and let $s$ be the coordinate on the $\R_{\ge0}$ or $\R_{\le0}$ factor. Then $\tild H$ is both $s$- and $t$-independent, $P$ is $s$-independent, and $\beta=wdt$ for some positive constant $w$ depending on the end.
 \item $d\beta\le0$ and $\beta|_{\partial\Sigma}=0$.
 \item\label{cd:negative derivative} Outside of a compact set, both $d^\Sigma\tild H\wedge\beta$ and $d^\Sigma P\wedge\beta$ are nonpositive.
 \item $P$ is globally bounded, and $\|X_P\|$ decays exponentially in the symplectization coordinate $\sqrt{\tild H}$ for any metric coming from some $J\in\mathcal J^\Sigma(M,\tild H)$.
\end{enumerate}
Finally, we suppose we have some $\Sigma$-parametrized $\hat\omega_M$-compatible almost complex structure $J$.

\begin{rmk}
 These conditions correspond individually to conditions we imposed on Floer data throughout the text, see in particular Definitions \ref{defn:Floer datum} and \ref{defn:Floer datum w/ cylinders}.
\end{rmk}

Set $H=\tild H+P$. 

Let $\Sigma$ be a punctured Riemann surface with labeled boundary, ends, and cylinders, and let $K$ be a Floer datum on $\Sigma$. We consider the space $\mathcal M$ of maps $u\colon\Sigma\to\hat M$ sending every $z\in\partial_i\Sigma$ to a point $L_i(z)$ and satisfying the inhomogeneous Cauchy-Riemann equation \ref{eq:gen Floer w/ cylinders}. Given a K\"ahler metric on $\Sigma$, define the \textbf{geometric energy} of such $u$ as
\[
 E^{geom}(u)=\int_\Sigma\lVert du-X_{H+P}\otimes\beta\rVert^2 dvol,
\]
where the metric on $\hat M$ is $\Sigma$-dependent and is obtained from $J$. This is independent of the choice of K\"ahler metric on $\Sigma$ and is in fact given by
\[
 E^{geom}(u)=\int_\Sigma\left(u^*\hat\omega_M-u^*(d^{\hat M}(H+P))\wedge\beta\right).
\]

We also define the \textbf{topological energy} of $u$ by
\[
\begin{aligned}
 E^{top}(u)&=\int_\Sigma\left(u^*\hat\omega_M-d(u^*(H+P)\beta)\right)\\
 &=E^{geom}(u)-\int_\Sigma\left(u^*(H+P)d\beta+u^*(d^\Sigma(H+P))\wedge\beta\right).
\end{aligned}
\]
\begin{lemma}\label{lem:E^geom E^top inequality}
 There is some constant $C\in\R$ depending only on $\Sigma$, $H+P$, and $\beta$ for which
 \[
  E^{top}(u)\ge E^{geom}(u)+C
 \]
 for all $u\in\mathcal M$.
\end{lemma}
\begin{proof}
 $(H+P)d\beta$ is nowhere positive, and $d^\Sigma(H+P)\wedge\beta$ is only positive on a compact subset of $\Sigma\times\hat M$.
\end{proof}
\begin{cor}\label{cor:E^geom E^top bound}
 The above constant $C$ is bounded below by $-\int_\Sigma\max_{\hat M}(d^\Sigma(H+P)\wedge\beta)$
 \qed
\end{cor}

We now examine the relation between action and topological energy . For any $u\in\mathcal M$ with $E^{geom}(u)<\infty$, $u$ converges at each interior puncture $\zeta_j$ to a 1-periodic orbit $x_j$ of $w_jX_{H+P}$ and at each boundary puncture $\zeta^k$ to a chord $\gamma^k$ of $w^kX_H=w^kX_{H+P}$, for appropriate 1-parameter specializations of $H$. Before we define the action, choose for each Lagrangian $L$ a primitive $f_L\in C^\infty(L)$ of the exact 1-form $\hat\lambda_M|_L$. For an orbit $x$, define
\[
 A(x)=\int_{S^1}\left(x^*\hat\lambda_M-wx^*(H+P)dt\right).
\]
For a chord $\gamma$, let $L_0$ and $L_1$ be the Lagrangians containing $\gamma(0)$ and $\gamma(1)$. Define
\[
\begin{aligned}
 A_0(\gamma)&=\int_{[0,1]}\left(\gamma^*\hat\lambda_M-w\gamma^*(H+P)dt\right)\\
 A(\gamma)&=\int_{[0,1]}\left(\gamma^*\hat\lambda_M-w\gamma^*(H+P)dt\right)+f_{L_0}(\gamma(0))-f_{L_1}(\gamma(1)).
\end{aligned}
\]
With this set up, we have the standard action-energy identity
\begin{lemma}\label{lem:action-energy identity}
 Every $u\in\mathcal M$ with $E^{geom}(u)<\infty$ satisfies
 \[
  E^{top}(u)=\hspace{-2mm}\sum_{\substack{\text{positive}\\ \text{cylindrical}\\ \text{ends }\epsilon_j}}\hspace{-2mm}A(x_j)+\hspace{-2mm}\sum_{\substack{\text{positive}\\ \text{strip-like}\\ \text{ends }\epsilon^k}}\hspace{-2mm}A(\gamma^k)-\hspace{-2mm}\sum_{\substack{\text{negative}\\ \text{cylindrical}\\ \text{ends }\epsilon_j}}\hspace{-2mm}A(x_j)-\hspace{-2mm}\sum_{\substack{\text{negative}\\ \text{strip-like}\\ \text{ends }\epsilon^k}}\hspace{-2mm}A(\gamma^k).
 \]
\end{lemma}
\begin{proof}
 Stokes's theorem.
\end{proof}
\begin{cor}\label{cor:action bound}
 Suppose $\Sigma$ has exactly one negative end $\epsilon_-$, either strip-like or cylindrical. Let $u\in\mathcal M$ be a finite-energy holomorphic curve converging at $\epsilon_-$ to an orbit or chord $y$. Then
 \[
  A(y)\le\hspace{-2mm}\sum_{\substack{\text{positive}\\ \text{cylindrical}\\ \text{ends }\epsilon_j}}\hspace{-2mm}A(x_j)+\hspace{-2mm}\sum_{\substack{\text{positive}\\ \text{strip-like}\\ \text{ends }\epsilon^k}}\hspace{-2mm}A(\gamma^k)+\int_\Sigma\max_{\hat M}(d^\Sigma(H+P)\wedge\beta)$.
 \]
 \qed
\end{cor}
